Report on the Advanced Linear Collider Study Group (ALEGRO) Workshop 2024

The workshop focused on the application of ANAs to particle physics keeping in mind the ultimate goal of a collider at the energy frontier (10\,TeV, e$^+$/e$^-$, e$^-$/e$^-$, or $\gamma\gamma$). The development of ANAs is conducted at universities and national laboratories worldwide. The community is thematically broad and diverse, in particular since lasers suitable for ANA research (multi-hundred-terawatt peak power, a few tens of femtosecond-long pulses) and acceleration of electrons to hundreds of mega electron volts to multi giga electron volts became commercially available. The community spans several continents (Europe, America, Asia), including more than 62 laboratories in more than 20 countries. It is among the missions of the ICFA-ANA panel to feature the amazing progress made with ANAs, to provide international coordination and to foster international collaborations towards a future HEP collider. The scope of this edition of the workshop was to discuss the recent progress and necessary steps towards realizing a linear collider for particle physics based on novel-accelerator technologies (laser or beam driven in plasma or structures). Updates on the relevant aspects of the European Strategy for Particle Physics (ESPP) Roadmap Process as well as of the P5 (in the US) were presented, and ample time was dedicated to discussions. The major outcome of the workshop is the decision for ALEGRO to coordinate efforts in Europe, in the US, and in Asia towards a pre-CDR for an ANA-based, 10\,TeV CM collider. This goal of this coordination is to lead to a funding proposal to be submitted to both EU and EU/US funding agencies. This document presents a summary of the workshop, as seen by the co-chairs, as well as short 'one-pagers' written by the presenters at the workshop.

==> contributions/PhilippePiot_old.tex <==
\vspace{1cm}
\section{Advances in SWFA R\&D for integration in linear colliders}\\
\addtocontents{toc}{\hspace{0.6cm}\textbf{\textit{P. Piot}}}
\subsection*{P. Piot}\\

\textit{Northern Illinois University, DeKalb Illinois 60115, USA \& Argonne National Laboratory, Argonne, Illinois 60439, USA}
\\
\\
The concept of structure wakefield acceleration (SWFA) offers a pathway to GV/m accelerating fields with operating frequencies ranging from X-band to THz. The implementation of SWFA can be based on collinear wakefield acceleration (CWA) or two-beam acceleration (TBA). CWA shares many features of the PWFA concept where a drive beam produced high-accelerating field experiences by a main bunch located propagating along the same path with the proper delay. TBA is unique to SWFA and uses a drive beam to excite high-power electromagnetic (EM) pulses in a power-extraction structure which are outcoupled and transferred to an accelerating structure used to boost the main-beam energy. TBA has the advantage of decoupling the beam dynamics of the drive and main beams at the expense of having two parallel beamlines with independent focusing, diagnostics, and other auxiliary components.   

To date, the SWFA community has primarily concentrated on a Linear Collider (LC) straw-person design utilizing the TBA implementation due to its maturity. A concept akin to CLIC design scaled to 26\,GHz was proposed in~\cite{Gai}. Meeting LC requirements entails producing an EM pulse peak power of 1\,GW in the power-extracting structure. While peak power close to 0.6\,GW~\cite{Picard} was achieved over the past three years, it is currently constrained by the quality and energy of available drive beams. Additionally, the staging of TBA was successfully demonstrated using X-band structures~\cite{Jing}. Recently, surface fields approaching 0.6\,GV/m were reached in a photoinjector powered by the TBA scheme~\cite{Tan}. The ability of TBA to generate high-peak-power short EM pulses, with durations less than 10\,ns at X-band frequencies, is key to achieving these high-peak fields. The short EM pulses significantly reduce breakdown rates and enable higher yields compared to klystron-powered structures. Comparable sub-GV/m peak fields were also obtained in other accelerating structures~\cite{Shao}. Over the next five years, a comprehensive TBA concept aimed at demonstrating the generation and acceleration of bright beams to 0.5\,GeV is planned, potentially driving a free-electron laser operating in the vacuum- or extreme-ultraviolet (V/EUV) regime~\cite{Piot}. 

The exploration of the Collinear Wakefield Acceleration (CWA) option for SWFA is also underway. Thus far, an integrated design of a multi-user FEL facility was proposed, which motivated the investigation of a single-stage CWA concept~\cite{Zholents}. Moreover, extensive research has been conducted on the topic of drive-beam shaping, resulting in the demonstration of a record transformer ratio of $\sim$5~\cite{missing}. Finally, efforts to study the transverse beam stability and mitigate the beam-breakup instability are actively underway, both theoretically~\cite{Baturin} and experimentally~\cite{Lynn,Lynn2}. An experimental program focused on developing an integrated CWA-based accelerating module capable of doubling the energy of the AWA accelerator in Argonne is currently in the planning phase. It should be also stressed that CWA implementation of SWFA shares many commonalities with PWFA, thereby offering opportunity for collaboration on the topics of shaped drive beam generation, and phase space manipulation and cooling of the electron and positron main bunches.   

Both the CWA and TBA concepts ultimately depend on the development of efficient numerical tools. A significant aspect of SWFA modeling involves designing structures with optimal RF performances and geometry to control the topology of the electromagnetic field. However, integrated simulation of the beam dynamics, particularly in CWA, is still lacking, with only a handful of particle-in-cell finite-difference time-domain computer programs incorporating electromagnetic boundaries and macroscopic properties relevant to SWFA (WARP-X~\cite{Tan2} being the exception). 

% References:  

% [1] W. Gai, et al., “Short-pulse dielectric two-beam acceleration”, J. Plasma Phys. 78, p. 339; DOI: 10.1017/S0022377812000037 (2012).   
% [2] J. Picard, et al., “Generation of 565 MW of X-band power using a metamaterial power extractor for structure-based wakefield acceleration”, Phys. Rev. AB 25, 051301; DOI: 10.1103/PhysRevAccelBeams.25.051301 (2022).  
% [3] C. Jing, et al., “Electron acceleration through two successive electron-beam-driven wakefield acceleration stages”, Nucl. Instr. Meth. A 898, p. 72; DOI: 10.1016/j.nima.2018.05.007 (2018). 
% [4] W.-H. Tan, et al., “Demonstration of sub-GV/m accelerating field in a photoemission electron gun powered by nanosecond X-band radio-frequency pulses”, Phys. Rev. AB 25, 083402; DOI: 10.1103/PhysRevAccelBeams.25.083402 (2022). 
% [5] J. Shao, et al., “Recent progress of short pulse dielectric two-beam acceleration”, in Proc. IPAC18; DOI: 10.18429/JACoW-IPAC2018-TUYGBE3 (2018).  
% [6] P. Piot, et al, “Development of a Compact Light Source using a Two-beam-acceleration Technique”, in Proc. ICFA FLS2023; DOI:10.18429/JACoW-FLS2023-MO4C2 (2023).  
% [7] A. A. Zholents et al. “A conceptual design of a compact wakefield accelerator for a high repetition rate multiuser x-ray free-electron laser facility”, in Proc. IPAC18, p. 1266, DOI:10.18429/JACoW-IPAC2018-TUPMF010 (2018).  
% [9] S. S. Baturin and A. Zholents, “Stability condition for the drive bunch in a collinear wakefield accelerator”, Phys. Rev. AB 21, 031301; DOI: 10.1103/PhysRevAccelBeams.21.031301 (2018).  
% [10] W. Lynn, et al., “Demonstration of transverse stability in an alternating symmetry planar dielectric structure", in Proc. Proc IPAC23, p. 1502, DOI: 10.18429/JACoW-IPAC2023-TUPA080 (2023).  
% [11] W. Lynn, et al., “Observation of skewed electromagnetic wakefields in an asymmetric structure driven by flat electron bunches", ArXiV:2308.09137; DOI: 10.48550/arXiv.2308.09137 (2024). 
% [12] W.H. Tan, et al., “Simulation Studies of Drive Beam Instability in a Dielectric Wakefield Accelerator”, in Proc. IPAC22, p. 645; DOI: 10.18429/JACoW-IPAC2022-MOPOMS012 (2022). 

==> mainWG1.tex <==
%\documentclass{cernrep}

%\usepackage{texnames}
%\usepackage[T1]{fontenc}

%\usepackage{graphicx}
%\usepackage{multirow}

%\pagestyle{plain}
%\begin{document}

%\title{%ANAR2017 DRAFT
%Summary Report for Working Group 1: Laser Wakefield Acceleration}
%
%\author{Arnd Specka$^{1}$, Daniel Gordon$^{2}$, and Carl B. Schroeder$^{3}$}
%\institute{$^{1}$\'{E}cole Polytechnique, CNRS-IN2P3, Palaiseau, France\\
%$^{2}$Naval Research Laboratory, Washington, DC, USA\\
%$^{3}$Lawrence Berkeley National Laboratory, Berkeley, CA, USA}

%\maketitle

\section{Introduction}

The laser wakefield accelerator (LWFA) is the most widely studied
advanced acceleration scheme and has demonstrated the highest
accelerating gradients to date (for a technical review of LWFA physics
and development see, for example~\cite{Esarey09,Malka12,Hooker13}). The wealth of results and the
constant budding of new research groups -- within and outside of
accelerator facilities -- has been made possible by the advent of
commercially available femtosecond lasers in the 100\,TW class -- and
now even in the PW class. The LWFA technique promises the highest
acceleration gradients but also has intrinsic challenges and
difficulties if one wishes to extrapolate existing research results to
a HEP collider design. An objective of the Workshop was to pinpoint the
scientific challenges and possible technological bottlenecks on the
road to an LWFA-based TeV e$^-$/e$^+$ collider and to suggest reasonable
near-term and mid-term milestones with the goal of defining a
long-term strategy. Working Group 1 gathered about 30 participants and
convened in four topical sessions, two discussion and two summary
sessions for a total of ten hours.
%The detailed agenda of the working
%group is shown in Appendix~\ref{appendix:program}.
The outcome and
identified milestones have been synthesized in a table in section~\ref{appendix:milestones}.

\section{State-of-the-art LWFA Experiments Relevant to HEP
Applications}

Presently, LWFA experiments accelerate electrons originating from the
background plasma itself. However, this is only for reasons of
experimental ease and of course there is no fundamental restriction
that other particles can be accelerated by an LWFA given these are
externally produced and pre-accelerated to relativistic energies. In
particular, in the context of high-energy physics, an LWFA is capable
of accelerating both electrons and positrons.

Reduced to its simplest expression, two numbers characterize the
discovery potential of a high-energy collider: center-of-mass energy
and luminosity. The center-of-mass energy is given by the sum of the
energies of the colliding e$^-$e$^+$ and determines the accessible range
of reactions in which production of unknown particles occurs or
metrology of recently discovered massive particles can be undertaken.
Luminosity can be assimilated to an average particle flux density and
determines the rate at which fundamental reactions occur in
collisions: the smaller the intrinsic probability of a given process,
the higher the luminosity has to be in order to be able to observe a
useful number of events. Luminosity in turn is determined by several
parameters: number of particles in one bunch (bunch charge), collision
repetition rate (bunch frequency) and beam size (emittance).

Past and present LWFA research has concentrated on both aspects,
aiming at ever higher energies and higher bunch charges. At the same
time, considerable effort has been made in improving the bunch quality
and reproducibility.

The progress on the energy frontier is illustrated in Figure~\ref{Fig1} where the LWFA beam energy gain from rest is shown as a
function of plasma density over one decade (2004-2014). As expected
from simple scaling laws, energy gain in a single LWFA stage increases
as the plasma density is reduced, and the acceleration length and
laser power are increased (not shown). The highest energy achieved so
far in an LWFA is 4~GeV over an acceleration length of 9\,cm using a
300\,TW Laser~\cite{Leemans14}. Achieving higher energy, while
maintaining a high gradient, will require staging multiple plasma
accelerators. Recent experiments in LWFA staging have transported and
injected an electron-beam generated in one LWFA stage into a second,
independently powered, LWFA stage~\cite{Steinke16}.

\begin{figure}
\centering\includegraphics[width=11cm]{fig1-wg1sum}
\caption{The progress on the energy frontier in a single LWFA stage
goes hand-in-hand with a decrease of plasma density. Dashed line is
$\Delta \mathcal{E} \propto 1/n$ scaling.}
\label{Fig1}
\end{figure}

Table~\ref{tab1} summarizes a non-exhaustive compilation of LWFA
performance achieved and observed by different groups in terms of the
critical beam parameters: energy, energy spread, normalized transverse
emittance (determines beam focusability and luminosity), bunch
duration, bunch charge and repetition rate. It is impossible here to
delve into the technical details and experimental intricacies;
however, in general, all of the cited results operated in strongly
non-linear regimes, with (natural, enhanced or assisted)
self-injection of plasma electrons and natural or assisted guiding of
laser propagation.


\begin{table}
\caption{LWFA performance}
\label{tab1}
\centering
\begin{tabular}{l|l|l}\hline\hline
Electron beam  & Experimentally demonstrated   &
References\\

 property  &  value(s)   &
\\
\hline
\hline
Peak energy
& 2\,GeV ($\pm$5\%, 0.1\,nC) & \cite{Wang13}  \\
&3\,GeV ($\pm$15\%, $\sim$0.05\,nC) & \cite{Kim13} \\
&4\,GeV ($\pm$5\%, 0.006\,nC)& \cite{Leemans14} \\
\hline
Energy spread &  5-10\% & [typical number\\
 &  &  many refs.]\\
& 1\% (at 0.01\,nC, 0.2\,GeV)& \cite{Rechatin09}\\
\hline
Norm. transverse & $\sim$0.1\,mm-mrad  &
\cite{Geddes08,Brunetti10,Plateau12,Weingartner12} \\
emittance & &  \\
\hline
Bunch duration & $\sim$ few fs &
\cite{Buck11,Lundh11,Heigoldt15,Zhang16} \\
\hline
Bunch charge & 0.02\,nC (at 0.19\,GeV $\pm$5\%)  & \cite{Rechatin09} \\
& 0.5\,nC (at 0.25\,GeV $\pm$14\%)  & \cite{Couperus17} \\
\hline
Repetition rate & $\sim$1\,Hz at $\sim$1\,GeV & [typical Ti:Al$_2$O$_3$
 system] \\
& 1\,kHz at $\sim$1\,MeV & \cite{He15,Salehi17,Guenot17} \\
\hline\hline
\end{tabular}
\end{table}

\section{Main Challenges to be Addressed in the Near-term and Mid-term Future}

The principal present-day challenges of plasma -- and in particular
laser-driven -- accelerators were identified, and strategies to
address them were discussed at the Workshop. Although programming of
realistic milestones will require intense, long-term work beyond
the time scale of a single two day workshop, a consensus could be
reached on which challenges should be addressed in the near-term
(e.g. five year) and mid-term (e.g. ten year) future. In the United
States, a roadmap for plasma-based accelerator R\&D has been developed
and reported in ~\cite{DOE-HEP-Roadmap16}. The challenges identified
at this Workshop are well aligned with ~\cite{DOE-HEP-Roadmap16}.
Realistic milestones would have to be combined and put into the
perspective of a global design effort in the long term (e.g. ten to twenty
years) whose contours are still to be defined precisely.

\subsection{Energy Efficiency}

Without energy recovery, the energy efficiency of a plasma
accelerator, i.e. the ratio of power in the beam to the consumed
electrical power, can be expressed as the product of two efficiencies:
wall-plug-to-driver and driver-to-beam. Plasma-based accelerator
concepts are frequently (and rightfully) criticized for the
excessively low energy efficiency. Indeed, in an acceptable collider
design, operation cost must not outrun significantly the construction
cost. For a collider, an overall energy efficiency of order $\sim$10\%
is required.

In this respect, laser-based concepts rank worst since the present
efficiency of high-peak-power laser drivers is three to four orders of
magnitude lower than RF drivers (klystrons) used in conventional
accelerator technology. The development of high-efficiency laser
drivers has been recognized as an absolute necessity, and is a
technological goal that is vigorously pursued in institutional and
industrial laser R\&D for reasons beyond advanced accelerator
research. In the long-term future, a wall-plug-to-laser efficiency of
the order of 50\% should be targeted in order to match the theoretically
achievable driver-to-beam efficiency of the same order, with
comparable depletion length and dephasing lengths.

Experimental and simulation evidence exist that show, at present,
the laser-to-beam efficiency could reach the order of 10\% in the
highly non-linear regimes at high plasma densities. The beam quality,
however, is rather poor under these conditions. Simulations advocate
that the driver-to-beam efficiency can be increased by optimizing the
beam loading using bunches with triangularly shaped longitudinal
current profiles.

As an alternative to using a single high-peak-power laser as a driver,
the concept of using optimally tailored laser pulse trains to excite
the plasma wave resonantly has been presented~\cite{Cowley17}. This
technique is particularly advantageous in the quasi-linear regime at
low plasma frequencies since it imposes less stringent requirements on
the laser spectral bandwidth.

\subsection{Stability}

In past experiments, the electron bunch parameters (peak energy,
energy spread, bunch charge, beam divergence) fluctuate strongly on
short and long time scales (shot-to-shot and day-to-day), and from
experiment-to-experiment for similar (or near-identical) conditions.
Although stability and reproducibility of electron beams have greatly
improved, LWFA produced beams do not yet approach the stability and
reproducibility of conventionally produced beams. The identification
and characterization of LWFA regimes of stable and reproducible
operation is now the main focus in novel accelerator R\&D. Further
progress requires the continuous development of reliable
diagnostics and an effort in performance calibration between research
groups. The development of high-repetition rate, e.g. kHz and beyond,
high-peak-power laser systems will enable feedback controls that
should greatly aid in improving stability and optimization.

\subsection{Bunch Charge}

Using self-injection in the highly nonlinear bubble regime,
the spectral bunch charge, i.e. the number of electrons per unit of
energy, is rather low. However, the spectral bunch charge is only one
of the key parameters, and owing to the short bunch duration and low
emittance, the six-dimensional beam brightness can be comparable or
better than state-of-the-art conventional sources. In addition, the
momentum acceptance of a typical beam transport and manipulation
system is generally limited to less than 1\%, limiting the bunch
charge. The spectral charge can be increased by triggered injection
methods and optimizing the beam loading.

\section{Towards a LWFA-based Collider}

Building on existing concepts for conventional linear e$^-$/e$^+$
colliders, a few salient challenges for LWFAs have been identified and
discussed. The maturity of existing studies on these issues range from
`close to completion' to `embryonic.' Development of an LWFA-based
e$^-$/e$^+$ collider design, fully integrating the collider subsystems with
the plasma accelerator, is a long-term R\&D effort. Many of the
collider subsystems (e.g. final focus, beam-delivery system, damping
and cooling systems, etc.) will have to be re-designed to be
compatible with (and take full advantage of) plasma accelerators. Work
on the LWFA-based collider subsystems is in the very early conceptual
stages.

\subsection{Step One: Building a Single-stage LWFA Injector}

In the near-term (i.e. next five years), LWFA experimental and computational
studies will have to concentrate on the consolidation and
improvement of beam parameters and accelerator performance. Therefore,
acceleration of plasma electrons seems the most accessible path on
this time scale at existing or upcoming facilities. The demonstration
of an LWFA-based source of femtosecond electron bunches in the energy
range of a few hundred MeV (e.g. 200\,MeV) was identified at the
workshop as a reasonable, benchmarkable goal. Tentatively, target
values for the main parameters have been defined. The LWFA should
deliver at least 100\,pC (10$^9$ electrons) in a stable manner:
fluctuations of the bunch charge should be at the few percent level,
energy dispersion and fluctuation $<$1\% and the pointing stability
better than 0.1\,mrad.

In the mid-term (i.e. next ten years), a plasma injector will have to
achieve all of these performance goals simultaneously, and go beyond
these target values. In the near term, however, it is realistic to
require that only some of these conditions (on duration, energy,
charge, energy spread and pointing) be fulfilled simultaneously.

Once the demonstration of a routinely delivered, high-quality beam of
electrons is demonstrated (at several facilities) this would open the
possibility to address the topics pertinent to HEP applications.



\subsection{Staging: Bunch Charge and Emittance Preservation}

Conventional linear accelerators achieve the highest particle energies by
stacking hundreds of so called RF units -- cavities powered by
klystrons -- with each acceleration stage providing a finite kinetic
energy increment. Also in plasma acceleration, staging is necessary
for high energy. As Figure~\ref{Fig1} shows, going to higher energy in a single
LWFA stage requires lower plasma density, which provides a lower
accelerating gradient (and longer acceleration length). To achieve
high beam energies at high accelerating gradients requires operating
many LWFA stages at moderate plasma density, each LWFA stage providing
a finite kinetic energy increment. For example, of the order of 100
stages would be required using an LWFA stage producing 10\,GeV energy
gain to reach TeV energy.

In the near term, a staging experiment should demonstrate acceleration
in two LWFA stages of more than 10\,cm length at a gradient higher than
0.1\,GeV/cm of an externally injected bunch, be it from an RF linac or
from an LWFA injector, for a substantial amount of charge. In the
mid-term, stages have to attain lengths of order 1\,m while preserving
all essential bunch qualities, and thus demonstrate scalability to
hundreds of stages.

\section{Positron Creation and Acceleration}

In the LWFA linear regime, positrons can be accelerated in the same
way as electrons by choosing a different injection phase in the plasma
wave. With non-linear effects, this symmetry no longer holds exactly,
and the above mentioned issues for electrons (emittance conservation,
optimal beam loading) have to be studied separately. In the
highly nonlinear bubble/blowout regime, the difference of the
behavior of electrons and positrons in the plasma wave becomes
extreme and high-quality positron beam acceleration is problematic.

Experimental studies of positron acceleration will become accessible as
soon as external injection in an LWFA stage is routinely achieved.
Since the necessary technologies for injection are likely to be
compact and potentially plasma-based, one can envisage a purely
laser-based positron acceleration experiment that could dispense with
conventional positron sources and RF accelerators.

In the near-term future, experimental demonstration of positron
acceleration should concentrate on developing methods for the creation
of femtosecond positron bunches using LWFA electron beams, and on
their injection into an LWFA stage in existing and upcoming laser
facilities. This will render possible the study of the acceleration
process for positron bunches (probably at low charge), and assess, for
example, emittance growth in the LWFA-accelerated positron beams in
the mid-term future.

Creating positrons from LWFA-generated electrons, either through
direct conversion on a target or through the intermediate step of
gamma-ray production, are subject to significant downselection. The
former method is easy to implement, but likely to result in very low
positron yields. The latter method proceeds along the line of proposed
schemes for positron production in future linear accelerator designs.
The idea of using a CO$_2$ laser for gamma production through
Compton scattering has been proposed~\cite{Yakimenko06}. Integrated
gamma sources combining an LWFA and Compton backscattering have already
been demonstrated energies well above the pair production threshold~\cite{Powers14}, and this method offers the possibility to create polarized radiation and, hence, polarized positrons via photon pair production.

For a collider application, positron bunches of similar quality
(charge, emittance, duration) as the electron beam are required. While
proof-of-principle experiments seem accessible at smaller laboratories and
laser facilities, it is likely that a full module test can only be
performed at accelerator laboratories able to provide the necessary
infrastructure, equipment and know-how.

\subsection{Polarization}

For the exploration of physics beyond the standard model with linear
e$^-$/e$^+$ colliders in the TeV energy regime, it is advantageous, if not
mandatory, to measure interaction cross-sections for well-defined
helicities of the initial state e$^-$/e$^+$s. Therefore, current linear
collider designs entail preparation and conservation of longitudinally
spin-polarized beams.

LWFA studies will have to address this issue both theoretically and
experimentally. Whereas the preparation of polarized beams can be
considered identical to conventional collider designs, the
conservation of polarization in the high gradients and the plasma
environment has to be studied in computer simulations in the
near-term future in order to identify the regimes where polarization
is preserved. (Initial studies indicate that electron polarization is
not destroyed~\cite{Vieira11}). Experimental investigation of
polarization conservation in LWFAs requires an accelerator lab
environment where polarized beams and possibly polarization analyzers
are available. Once external injection of an ultra-relativistic
electron beam in an LWFA stage is mastered, a dedicated experiment
should investigate the effect of plasma acceleration on the beam. Due
to the complexity of this endeavor it is likely that this study can
only be carried out in the long-term future, and would be integrated
in a global design effort for a plasma based collider.

In the near and mid-term future, ultra-high gradient acceleration in
wakefields might bear opportunities to study novel, plasma-based
techniques for creating polarized electron and/or positron beams.

\section{Long-term View for the HEP Application of LWFAs}

Designing a HEP collider follows a well-defined workflow: physics
requirements dictate the properties of the beams at the interaction
point and collider parameters such as luminosity. These parameters and
detector constraints determine the beam delivery system and final
focus, which in turn determines the linear accelerator itself.
Finally, the electron and positron source complexes will be defined
correspondingly.

The spatio-temporal properties of LWFA-generated beams differ strongly
from conventional beam properties. Therefore, it is likely that a
design study of a LWFA-based linear collider will have to be strongly
adapted to these properties. For example, the chromaticity of LWFA
beams would call for several kilometer long beam delivery systems, if
the existing design for CLIC would be carried over to LWFA beams. If
-- despite all expected improvements in LWFA beam quality -- one has
to live with a larger beam chromaticity, it will be necessary to
redesign the machine--detector interface completely anew.

A preliminary collider design study has to be initiated in the very
near future, aiming for a conceptual design report (CDR) in the
mid-term and a technical design report (TDR) at the 15 year horizon.
Such a coordinated effort will be beneficial for defining priorities
and concentrating research effort on identified bottlenecks.

\section{Required Technological Developments}

\subsection{High Average and Peak-power Laser Drivers}

Presently, the principal hurdles on the path towards an LWFA-based
accelerator are the low repetition rate and the low energy conversion
efficiency of the laser itself. This may seem paradoxical, since most
of the emblematic results have been achieved using lasers and, in
particular, femtosecond lasers that use titanium-doped sapphire
(Ti:Al$_2$O$_3$) as the gain medium. Ti:Al$_2$O$_3$ lasers, operating
around 0.8~$\mu$m wavelength, support ultrafast laser pulses down to
tens of femtoseconds with high energy per pulse and are the preferred laser for
plasma acceleration experiments. However, repetition rates of these
laser systems range from 1 to 10\,Hz. Even with the development of
suitable pump lasers and thermal management, it is considered unlikely
that Ti:Al$_2$O$_3$ laser technology will offer the possibility to
increase the repetition rate $>$kHz, owing to the large quantum defect
that results in an inherently low efficiency.

Lasers for an LWFA-based collider would have to achieve hundred kW
average powers with high efficiency. In order to attain these high
average and high-peak-power laser systems in the long-term,
exploration and development of alternative laser technologies has to
be pursued vigorously today. One possible approach is to rely on
coherent beam combining using multi-core fibers. This requires
coherent temporal, spatial and spectral stacking, of pulses produced
by diode-pumped fiber lasers. Such lasers have, potentially, very high
wall-plug efficiency (approaching 50\%) and could offer compact, very-high-power systems with tens to hundreds of kW average power.

In the mid-term, short-pulse, high-intensity lasers with repetition
rates of 1\,kHz (kW average power) are technically feasible, and
development of such laser systems is a critical step toward HEP
applications.

\subsection{Meter-length Plasma Structures at High Repetition Rates}

Present LWFA experiments explore a wide variety of accelerating plasma
structures of different degrees of complexity, such as the popular
supersonic gas jets (few millimeters length) and capillary
gas discharge channels (few centimeters length), but also gas cells and
hollow capillaries. The usage of a laser as the plasma wave driver
brings about the further constraint that the plasma has to guide the
focused laser and keep it collimated to counteract its tendency to
diffract.

In order to achieve a substantial energy gain, it is mandatory to
create plasma structures that will provide the accelerating field over
distances close to the depletion and/or dephasing length. In addition
to increased length, detailed tailoring of the plasma, both
longitudinally (for tapering and higher efficiency) and transversely
(for laser guiding) is required.

At the same time, these plasma sources will have to operate at
increasing cycle rates, above 10\,Hz in the near-term future, and up to
kHz in the mid-term future. These higher operation rates will enable
stability studies and implementation of efficient feedback loops. The
collider application will require plasma structures operating at
repetition rates of tens of kHz.

\subsection{Inter-stage Transport and Compact Laser In--Out Coupling}

In a staged accelerator, particular attention has to be given to
the way the laser is coupled into and out from the accelerating
plasma structures. At the same time, the electron or positron beam has to be
matched from one stage to the other. In order to maintain a high
average accelerating gradient, it is mandatory not to dilute the high
gradient that one will realize in the plasma stage by squandering the
space between stages. Plasma mirrors offers the possibility of compact
coupling of lasers between stages and development of plasma mirror
technology at high repetition rates is required.

Moreover, inter-stage charged particle beam transport has to preserve
the beam qualities, in particular charge and emittance. R\&D on
compact e-beam transport systems, possibly plasma-based, are also
required.

\subsection{Plasma Diagnostics}

In the near term, shot-by-shot plasma diagnostics, such as high-resolution imaging of the wakefield structure are necessary in order to
characterize regimes and conditions that allow stable and efficient
acceleration. In the mid-term, these will have to be coupled, at high
repetition rate, in a feedback loop to provide necessary
stabilization. In the long term, full four-dimensional imaging of
the plasma structure is desired.

\subsection{Electron Beam Diagnostics and Feedback}

In the near term, the characterization of the LWFA beams should be
improved. In particular, the reliable and precise measurement of the
bunch duration and of the transverse emittance are tasks that should
be given highest priority. Since repetition rates will be low in the
near term, it will be necessary to develop new single-shot measurement
techniques operating in ranges where conventional techniques are
expected to fail. Also, an effort to intercalibrate metrology methods
employed by different research teams will be beneficial for the
understanding of LWFA mechanisms and their optimization. In the
mid-term, it will be required to improve the metrology to measure
correlations between beam parameters, e.g. transverse (slice) and
longitudinal emittance, and to integrate these into a feedback loop to
stabilize actively the beam quality.

\section{Conclusions of the Working Group and Outlook}

Designing and actually building a plasma-based collider will be a
challenging task, calling on scientific competencies and technical
skills from many disciplines. Thus it is likely that this endeavor can
only be undertaken in the framework of a large, potentially worldwide
collaboration. On the other hand, the wealth of scientific results and
the worldwide budding of laser facilities documents that the
relatively young field of plasma accelerators is still in the
exploratory and discovery phase.

Future R\&D for a TeV-scale HEP collider is not the only application
of LWFA technology, and coordinated efforts exist for other
applications, e.g. 5$^{\mathrm{th}}$ generation X-ray light sources. While many
future studies will be carried out in smaller laboratories or laser
facilities, the community has to take the intermediate step to
demonstrate that LWFA technology can be employed to build a reliable
accelerator for applications. Design efforts like EuPRAXIA are
precisely aiming at proposing a dedicated facility~\cite{Walker17}.

It is illusory to believe that a full LWFA-based collider design or
any other plasma technique will be possible without a coordinated
effort accomplished by a large international community. It is
necessary to start preliminary design studies in the near future,
which will provide valuable guidelines for the research activities
already underway.
\clearpage

%\newpage
%\appendix

%\section{Program of Working Group 1 (LWFA)}
%\label{appendix:program}
%\begin{figure}[h!]
%\includegraphics[width=15cm]{ANAR-WG1-Program}
%\end{figure}

\clearpage

\section{Table of Scientific Challenges and Milestones}
\label{appendix:milestones}

\begin{tabular}{|l|l|l|l|}
  \hline
\hline
 Scientific challenges & \multicolumn{3}{|c|}{Milestones}
\\
   \hline
 & Near term  & Mid term  & Long term \\
  & (5 years) & (10 years) & (20 years)\\
  \hline
\hline
{\bf fs e-beam injector}  & 2 of 5  & 5 of 5  & 5
of 5
\\
Peak energy $>$200\,MeV & conditions & conditions &  conditions

\\
$\bullet$ energy stability: $ \Delta$E$_0$/E$_0 < $1\% & demonstrated & demonstrated&  with
 \\
 $\bullet$ energy spread: $\Delta$E/E < 2\% &&& beam shaping
 \\
 $\bullet$ charge: Q > 100\,pC &&&
 \\
 $\bullet$ charge fluctuation: $\Delta$Q/Q < 2\% &&&
 \\
 $\bullet$ pointing: $\Delta \theta<$0.1\,mrad &&&
\\
\hline
Repetition rate (experiment)&	10\,Hz &	100\,Hz	& 1\,kHz
\\ \hline
Laser repetition rate (laser)&	$>$10\,Hz& $>$100\,Hz&$>$1\,kHz
\\ \hline
Laser energy efficiency (laser)	& $>$1\% &$>$10\% & 50\%
\\ \hline
Laser beam quality &	$>$90\%   &&
\\
& energy in mode &&
\\ \hline
Scalable single stage  &	$>$10\,cm, 10 Hz &	1\,m, 100\,Hz &	1\,m, 1\,kHz
\\
(0.1\,GeV/cm) &&&
\\ \hline
Staging & $\sim$unity charge &  Scalability &
\\
& throughput, & (multi-staging) &
\\
& emittance  &&
\\
&  preservation &&
\\ \hline
Positron acceleration &	Identify and test &	Accel.\ demo.\
&	Parity with
\\
& injection method & (low $\epsilon_n$  &  electrons
\\
& & and $\Delta$E/E) &
\\
\hline
Fluctuations  &	Q, $\Delta$E, E$_0$, $\Delta \theta$ &Active control   &	All factors
\\
and feedback control & & of multiple & 1.01
\\
 & &  fluctuations&
\\
\hline
Efficient beam loading &	Ramped or &&
\\
(longitudinal bunch shaping) &  multi-pulses &&
\\ \hline
Diagnostic resolution &	fs resolution, & Energy/phase  &
\\
(bunch length and emittance) & $\epsilon_n  =$ 0.1\,mm-mrad  &
correlation, &
\\
 &  &
 single
shot &
\\ \hline
Multi-bunch acceleration & Generation,  &
Acceleration&
\\
&separation control &&
\\ \hline
%
Collider parameter (re)definition &  \multirow{3}{*}{Design study} &
\multirow{3}{*}{CDR} & \multirow{3}{*}{TDR}
\\ \cline{1-1}
BDS/FF design &&&
\\ \cline{1-1}
LWFA collider baseline design &&&
\\
\hline\hline
\end{tabular}

%\end{document}



==> mainWG3.tex <==
%\documentclass{cernrep}
%
%\usepackage[usenames, dvipsnames]{color}
%\begin{document}
%\title{Summary Report for Working Group 3:\\Structure-based Wakefield Accelerators}
%\author{P. Craievich~$^1$, P. Piot~$^{2,3}$, J. G. Power~$^4$}
%\institute{$^1$~Paul Scherrer Institut, 5232 Villigen, Switzerland \\
%$^2$~Northern Illinois University, DeKalb IL 60115, USA\\
%$^3$~Fermi National Accelerator Laboratory, Batavia, IL 60510, USA \\
%$^4$~Argonne National Laboratory, Argonne, IL 60510, USA }
%
% \begin{abstract}
% The working group `Structure-based Wakefield Accelerators' at the 2017 Advanced and Novel Accelerators  for High Energy Physics  Roadmap (ANAR17)  workshop  focused on beam-driven acceleration using solid-state assisting media such as dielectric-lined or corrugated waveguides and advanced electromagnetic accelerating structures.
% \end{abstract}
%\maketitle
%
\section{Introduction}
In structure-based wakefield accelerators (SWFAs) electromagnetic wakefields are excited in a solid-state structure by a charged particle bunch (the `drive' bunch). The structures are designed to support a strong axial electric field to accelerate a following `main' bunch. SWFAs can be implemented in a collinear wakefield accelerator (CWA) or a two-beam accelerator (TBA) configuration; see Figure~\ref{fig:tba}.
%
\begin{figure}[ht]
\begin{center}
\includegraphics[width=13cm]{cwaVstba.pdf}
\caption{Collinear wakefield accelerator (CWA) (a) and two-beam accelerator (TBA) schemes (b) configurations associated with structure-based wakefield accelerators.}
\label{fig:tba}
\end{center}
\end{figure}
%
In the former approach the drive and main bunches follow the same path while in the latter scheme the fields excited by the drive bunch are coupled to another structure that accelerates the main beam in a parallel beamline. The CWA is appealing as it only requires one beamline but presents challenges as the beamline lattice has to accommodate the drive- and main-beam dynamics. An important feature of SWFA is its indifference to the particle species: in the context of an e$^-$/e$^+$ ALC, it is anticipated that a drive electron bunch will produce wakefields adequate for acceleration of main electron and positron bunches accelerations.

The four main topics discussed in our working group included ($i$) the electromagnetic structures mediating the wakefield interaction, the beam dynamics of the $(ii)$ drive and $(iii)$ main beam and $(iv)$ the possible staging of `SWFA accelerating modules' to form high-energy beams.

The frequencies associated with the accelerating mode(s) supported by the structure typically range from the GHz to THz. Higher frequencies favor a higher shunt impedance (which increases the attainable accelerating gradients) but yield more stringent requirements on the beam emittances. The structures  proposed so far range from simple dielectric lined or corrugated waveguides to more advanced cavities. The later designs offer a better control over the electromagnetic field configuration at the expense of complexity (and cost).

The drive beam is accelerated to the required energy via  klystron-powered conventional cavities and typical wall-plug-to-drive-beam efficiency is in excess of 50\%. Likewise, temporally shaping the drive beam can enhance the transformer ratio ${\cal R} \equiv E_+/E_-$, where $E_+$ (resp. $E_-$) is the maximum decelerating field (resp. accelerating field) amplitude within the drive bunch (resp. available to the main bunch)~\cite{bane}. Additionally, tailoring the bunch transverse distribution can accommodate compact multi-channel structures where the drive and main beams travel in separate channels.

The main-beam specifications require a full design of the ALC. It is however conceivable that the main beam would be produced in a conventional high-brightness electron source coupled to a conventional accelerator for acceleration up to sufficient energy for radiation cooling in a damping ring. The subsequent acceleration of the main beam in the SWFA should mitigate sources of transverse emittance dilution.

Finally, an important aspect of SWFA is its straightforward staging: structures can be powered by the same drive beam in stages and the main-beam energy can be incremented.

In the following sections we present, for each of the identified topics, the current state of the art and identify areas where R\&D will likely be needed. We  conclude by providing a general roadmap discussed during the workshop.
%
\section{State of the Art}
\subsection{Structures}
The development of structures capable of supporting intense accelerating fields from a drive beam is an active research area. High-peak fields can be attained by using small-aperture structures which limit the drive-beam bunch charge thereby requiring  shorter drive bunches to produce the needed peak current. In addition to supporting high accelerating gradients, the structures must be operationally robust and have acceptable breakdown rates. Over the last two decades SWFAs have essentially focused on the use of dielectric lined waveguide (DLWs)~\cite{gai}. However potential limitations associated with DLW structures (e.g. multipacting and recently observed  `metallization' effects) along with developments in photonics have motivated further research on metallic structures.
%
%
Over the past few years ${\sim}100$~MV/m accelerating fields in GHz structures and sub-GV/m fields have been inferred in some experiments with THz-regime dielectric structures~ and \cite{thompson,oshea} have been demonstrated for several types of structure.  Additionally, various breakdown tests on metallic and dielectric structures have been performed~\cite{dalforno1,antipov3}. The availability of short bunches (short enough to drive structures operating at THz frequencies) at several facilities has facilitated SWFA experiments aimed at investigating acceleration and breakdown rates~\cite{dalforno1}. Finally, more advanced  structures based on plasmonic effects or meta-material properties are also being investigated and are expected to better control the supported field distribution (e.g. to suppress of harmful modes).
%
\subsection{Drive Beam }
%
One important topic associated with the drive beam is the need to tailor its spatio-temporal distribution (a need shared with PWFA)~\cite{bane}. Likewise, small beam misalignments in the SWFA result in beam disruption due to the beam break-up instability~\cite{bbu} induced by the possible excitation of transverse wakefields.
The formation of drive beams with tailored temporal distributions has progressed over the last decade owing to advances in phase-space manipulations. Some of the structures being proposed for CWA application incorporate multiple beam channels where one (or more) drive beam(s) and the main beam (e.g. a coaxial structure requires a annular-shaped drive beam with a main beam in its center) are injected. Likewise the possible use of asymmetric structures, e.g. to accommodate the required flat main beam, may require the production of drive beams with large transverse emittance ratios. Therefore transverse shaping of the drive bunch is sometime necessary. This type of shaping has been demonstrated at several facilities using photoemission electron source with parameters comparable to the ones foreseen for the drive beam electron source of a future ALCs. Precise shaping can be obtained by tailoring the photocathode laser pulse transverse distributions while large transverse emittance ratios `flat' beams have been obtained using linear manipulations.
Several temporal shaping schemes have been proposed the past decade including the possible use of laser shaping~\cite{lsrshaping}, transverse-to-longitudinal phase-space exchanger~\cite{eex3} or exploiting non-linear correlations introduced in the longitudinal phase space using aberration-controlled beamlines~\cite{england}, multi-frequency linacs or longitudinal wakefields~\cite{andonianshaping}.  Overall, the drive beam shaping has benefited from a strong interest and critical proof-of-principle experiments have been performed at available facilities.
A critical aspect associated with the drive beam regards its subjectiveness to the single bunch beam break-up (SBBU) instability.  This instability arises from misalignment in the SWFA structures and leads to a cumulated time-dependent kick which can eventually result in beam losses. High-frequency (THz) SWFAs are especially prone to SBBU and mitigation techniques devised for conventional linacs~\cite{bns} are being adapted to SWFAs. The standard SBBU mitigation technique (known as BNS damping) limits the maximum accelerating field for a given SWFA operating frequency~\cite{li_bbu}.
%
\subsection{Main Beam}
%
The required center of mass energy, T, and luminosity, L, set the main beam parameters, specifically its transverse normalized emittance, $\gamma\varepsilon$, and average power, P (or current I).  Thorough studies of the main beam parameters have not been performed for the SWFA schemes with the notable exception of CLIC.  The 3\,TeV CLIC LC design~\cite{clic} requires T/2 $=$ 1.5\,TeV, P $=$ 14\,MW, $\gamma\varepsilon=$ 77~nm-rad and I $=$\,$\mu$A. SWFA GHz schemes can take advantage of the CLIC main beam studies while THz schemes are lacking even a strawman design. It is however expected that THz SWFA will put stringent requirement on the emittances [${\cal O}$(nm)] requiring the development of ultra-low emittance e$^+$ and e$^-$ sources.  The development of such an e$^-$ source has recently begun~\cite{nanni}.
%
\subsection{Staging}
%
In principle, there are no fundamental physics limitations to staging in SWFA. To date, only a simplified version of staging was demonstrated for TBA in the GHz-regime~\cite{AWA1} where the drive beam was sent through both stages and a high brightness, 1\,nC main beam was accelerated with a field of 100 MV/m in successive stages.
%
\section{Roadmap}
\subsection{Structures }
The technical challenges for the dielectric lined waveguides for achieving the SWFA roadmap milestones can be summarized in two main topics: high electric field (>GV/m) can induce metallization of the dielectrics through non-adiabatic process~\cite{oshea} and the multipactor effect in long pulse dielectric lined waveguides can limit the RF power in the power extractor. Actually, the metallization of the dielectric has an implication for the dielectric accelerator design, i.e. field exclusion from dielectric (shape) and choice of the material. Multipactor can be suppressed with solenoid and further effort will be necessary to investigate other suppression techniques.
However, it should be noted that several laboratories have developed  technologies required for accelerating structures including, e.g. high-gradient, high-order mode suppression, high efficiency, transverse wakefield damping, RF breakdown mitigation, broadband impedance matching. We foresee that the future R\&D will focus on developing full-featured, dielectric and metallic structures that integrate all of these technologies, in order to reach higher gradients. Some advanced structures discussed included photonic band gap (PBG) structures~\cite{simakov}, metallic meta-materials (MTMs),  `dielectric-assist' accelerators (DAAs)~\cite{satoh}, photonic topological insulators (PTIs)~\cite{pti}, coaxial dielectric wakefield accelerator~\cite{coax}. Finally, the use of electromagnetic wakefield amplification by an active medium was also presented~\cite{levi2}.

\subsection{Drive Beam}
We foresee the drive beam R\&D to focus on beam shaping, general beam dynamics to control the SBBU instability and the requirement of a low-emittance high-charge injector to produce the require beam. \\
%
{\bf Longitudinal bunch shaping:} The recent investigation of improved shapes considering the multiple modes that can be excited by the drive beam in a structure should be refined via numerical simulations. In the near term, the compromise between optimal and practically achievable shapes should be understood via simulations for given structure designs. In a short-to-medium term, beamlines capable of forming the most promising shapes should be devised and experimentally demonstrated. In the medium term, it is expected that an experiment to demonstrate a significant transformer ratio with a temporally shaped bunch should be performed. \\
%
{\bf Transverse shaping:}  Tailored transverse beam distribution combined with temporal shaping should be pursued in the longer term. Some transverse shapes, e.g. annular beams, can be subject to instabilities that should be investigated and possibly mitigated. \\
%
{\bf Electron sources:}  As high gradient will be attained in SWFA operating in the THz regime, the development of adequate electron sources capable of providing the required low emittance is a important step. We note that such a development is synergistic with R\&D in the free-electron laser (FEL) community so that on-going development will benefit to future LCs. \\
%
{\bf SBBU control:} The investigation of SBBU via numerical simulation should be continued and supplemented by experiments for the cases of cylindrical dielectric lined waveguides (short term), planar dielectric and novel structures (mid term). For the latter case the use of longitudinally shaped flat beam should be explored.
%
\subsection{Main Beam}
%
The roadmap for the main beam R\&D has similar categories as the drive beam but with different goals.  \\
%
{\bf Longitudinal bunch shaping:} A critical issue for the LC is its site power requirement (e.g. CLIC Site Power is 600\,MW) due to the relatively low drive--main beam efficiency (26\%) as limited by beam loading and the energy spread requirement at the IP. Recent studies have shown~\cite{AWA1} that temporally shaping the main beam can significantly increase this efficiency potentially leading to $\sim$50\% reduction in site power. This would benefit all SWFA (and PWFA) schemes.  We recommend numerical studies in the near term, possibly supplemented by  experimental validation in the medium term. \\
%
{\bf Transverse shaping:}  This is almost identical to the drive beam transverse shaping since both beams often travel through the identical structure, as in the case of a planar waveguide.  However, in some cases, such as a coaxial structure,  the main beam requires no transverse shaping. Regardless of the structure, a flat beam is needed at the IP.\\
%
{\bf Electron and positron sources:} There is a dearth of main beam e$^-$ source development in the THz regime and no e$^+$ development so research here is needed on all time scales.  GHz sources are again relatively mature using the damping ring approach. Similarly to the drive beams, the electron sources R\&D within the FEL community will be beneficial. \\
%
{\bf Luminosity at the IP:}  Strawman designs should be completed in the near term. GHz-regime concepts have strawman designs but THz-regime have none so far. One makes different trade offs between emittance, current and repetition rate for the GHz and THz frequency regimes. A THz LC operated at a lower charge per bunch would use a higher repetition rate to deliver the same current. However, because the luminosity is given by L$\propto\frac{P}{\sqrt\epsilon}$ the power (or beam) requirements could be reduced if the emittance was lowered.  In the medium term, the strawman designs should be subjected to start-to-end simulations that consider emittance preservation to the IP including BBU, etc.  In particular, the CWA scheme must examine the effect of the drive beam wakefield on the stability of the main beam.

%
\subsection{Staging}
As stated above, there are no fundamental limitations to staging in SWFA but many technical challenges are anticipated.  Staging for the CWA scheme requires proper handling of the drive transverse jitter since the drive beam offset will generate transverse wakefields that could cause the emittance degradation or loss of the main beam. We recommend tolerance studies of the impact drive beam position stability on the main beam in the near term.  A second challenge is that staging in the THz regime will require femtosecond-scale stability to control the arrival time jitter.  This potential temporal stability issues should be studied in the medium term.  In the medium to long term, attempts should be made to experimentally demonstrate staging in the CWA THz regime.

\section{Outlook}
SWFAs are appealing for a e$^-$/e$^+$ LC. The scheme enjoys active on-going development of wakefield structures and will leverage  R\&D on electron-beam shaping and high-brightness electron sources being actively explored for other applications of electron accelerators (e.g. free electron lasers). The roadmap toward an engineering design of a SFWA-based LC  will first require the selection of an acceleration scheme (CWA versus TBA) which will depend on advances in drive beams (SBBU control and distribution tailoring). In parallel we foresee the process of identifying  wakefield structures to be twofold. First, a baseline design of an SWFA collider could be formulated by selecting the structure geometry (cylindrical versus planar) and material (dielectric versus metallic). In parallel to a baseline design based on `conventional' structures, R\&D on advanced structures should continue and could be possibly incorporated into an improved LC  design. The main beam will most likely be generated following a scheme identical to current LC design (e.g. initial acceleration in a conventional linac for radiation cooling in a damping ring). However on-going research in high-brightness injectors and advanced phase-space manipulation could alleviate the need for a damping ring in an improved design.

As a concluding remark we should point out that the research on drive beam shaping for enhanced transformer ratio is synergistic with the PWFA concept. Likewise, the development of advanced structures share similarities with R\&D related to DLA scheme.

%\bibliography{bibWG3}

%\begin{thebibliography}{99}
%\bibitem{bane} K. L. F. Bane, et al., SLAC-PUB-3662 (1985)
%\bibitem{gai}  W. Gai, et al., Phys. Rev. Lett. {\bf 61}, 2756 (1988)
%\bibitem{thompson} M. C. Thompson et al., Phys. Rev. Lett.  {\bf 100}, 214801 (2008)
%\bibitem{oshea} B. D. O'Shea, et al., Nature Communications {\bf 7}, 12763 (2016)
%\bibitem{dalforno1} M. Dal Forno et al., Phys. Rev. Accel. Beams {\bf 19}, 011301 (2016)
%\bibitem{antipov3} S.P. Antipov et al., Diamond and Related Materials 54 (2015)
%\bibitem{bbu} A. Chao, {\em Physics of Collective Instabilities in High-Energy Accelerators},  Wiley Series in Beams \& Accelerator Technologies, John Wiley and Sons (1993)
%\bibitem{eex3} G. Ha, et al., Phys. Rev. Lett. {\bf 118}, 104801 (2017)
%\bibitem{lsrshaping} G. Penco, et al., Phys. Rev. Lett. {\bf 112}, 044801 (2014)
%\bibitem{england} R. J. England, et al. Phys. Rev. Lett. {\bf 100}, 214802 (2008)
%\bibitem{andonianshaping} G. Andonian, et al., Phys. Rev. Lett. {\bf 118}, 054802 (2017)
%\bibitem{bns} V. Balakin, et al., in Proc. of the 12th Int. Conf. on High Energy Accel. (Fermilab), p. 119 (1983)
%\bibitem{li_bbu} C. Li, et al., Phys. Rev. ST Accel. Beams {\bf 17}, 091302 (2014)
%\bibitem{clic} CLIC Conceptual Design Report, CERN-2012-007 (2012)
%\bibitem{nanni} E. Nanni, et al., in the Proc. of the 2017 Int. Part. Accel. Conf. (IPAC2017), p. 3884 (2016)
%\bibitem{AWA1} J. Shao, et al., in Proc. of the 2017 Int. Part. Accel. Conf. (IPAC2017), p. 3305 (2017)
%\bibitem{simakov} E.I. Simakov et al., Phys. Rev. Lett. {\bf 116}, 064801 (2016)
%\bibitem{satoh} D. Satoh, et al., Phys. Rev. Accel. Beams {\bf 19}, 011302 (2016)
%\bibitem{pti} T. Ma, et al., Phys. Rev. Lett. {\bf 114}, 127401 (2015)
%\bibitem{coax} G.V . Sotnikov, et al., Proc. of 2011 Part. Accel. Conf., New York, NY, USA, MOP112
%\bibitem{levi2} Z. Toroker and L. Schaechter, Phys. Rev. ST Accel. Beams {\bf 18}, 071301 (2015)
%
%\end{thebibliography}



%\end{document}

